Accurate Weakly Supervised Deep Lesion Segmentation on CT Scans: Self-Paced 3D Mask Generation from RECIST

Volumetric lesion segmentation via medical imaging is a powerful means to precisely assess multiple time-point lesion/tumor changes. Because manual 3D segmentation is prohibitively time consuming and requires radiological experience, current practices rely on an imprecise surrogate called response evaluation criteria in solid tumors (RECIST). Despite their coarseness, RECIST marks are commonly found in current hospital picture and archiving systems (PACS), meaning they can provide a potentially powerful, yet extraordinarily challenging, source of weak supervision for full 3D segmentation. Toward this end, we introduce a convolutional neural network based weakly supervised self-paced segmentation (WSSS) method to 1) generate the initial lesion segmentation on the axial RECIST-slice; 2) learn the data distribution on RECIST-slices; 3) adapt to segment the whole volume slice by slice to finally obtain a volumetric segmentation. In addition, we explore how super-resolution images (2~5 times beyond the physical CT imaging), generated from a proposed stacked generative adversarial network, can aid the WSSS performance. We employ the DeepLesion dataset, a comprehensive CT-image lesion dataset of 32,735 PACS-bookmarked findings, which include lesions, tumors, and lymph nodes of varying sizes, categories, body regions and surrounding contexts. These are drawn from 10,594 studies of 4,459 patients. We also validate on a lymph-node dataset, where 3D ground truth masks are available for all images. For the DeepLesion dataset, we report mean Dice coefficients of 93% on RECIST-slices and 76% in 3D lesion volumes. We further validate using a subjective user study, where an experienced radiologist accepted our WSSS-generated lesion segmentation results with a high probability of 92.4%.

==> figures/visual_examples.tex <==
%!TEX root=../main.tex

\begin{figure*}[t]
\begin{center}
\setlength{\fboxsep}{0pt}
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/good_select/003036_01_4_201.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/good_select/001742_01_5_77.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/good_select/003406_01_4_158.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/good_select/000700_01_2_46.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/good_select/002143_01_2_45.png}} \hfill 
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/good_select/000122_01_7_50.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/good_select/004180_01_2_65.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/good_select/003211_02_3_552.png}} \\[2mm]
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/bad_select/000020_04_4_143.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/bad_select/000923_02_4_97.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/bad_select/002574_01_4_119.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/bad_select/000374_06_3_318.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/bad_select/000760_07_2_26.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/bad_select/001983_02_2_54.png}} \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/bad_select/002788_01_6_49.png}}  \hfill
 \fbox{\includegraphics[width=0.11\linewidth, height=0.11\linewidth]{figures/segments/bad_select/001217_02_2_100.png}} 
\end{center}
\caption{Visual Examples of accepted and rejected lesion segmentation examples from the subjective user study. The \textbf{first row} presents good cases that are accepted by both observers. In the \textbf{second row}, failed cases (rejected by both radiologists) are shown. The red curves delineate segmented lesion boundaries. The under-segmented lesion regions are illustrated by yellow arrows and the over-segmented healthy tissue areas are indicated by blue arrows. Better viewed in color version.}
\label{fig:visual-example}
\end{figure*}

==> sections/abstract.tex <==
%!TEX root=../main.tex

Volumetric lesion segmentation via medical imaging is a powerful means to precisely assess multiple time-point lesion/tumor changes. Because manual 3D segmentation is prohibitively time consuming and requires radiological experience, current practices rely on an imprecise surrogate called response evaluation criteria in solid tumors (RECIST). Despite their coarseness, RECIST marks are commonly found in current hospital picture and archiving systems (PACS), meaning they can provide a potentially powerful, yet extraordinarily challenging, source of weak supervision for full 3D segmentation. Toward this end, introduce a convolutional neural network based weakly supervised self-paced segmentation (WSSS) method to 1) generate the initial lesion segmentation on the axial RECIST-slice; 2) learn the data distribution on RECIST-slices; 3) adapt to segment the whole volume slice by slice to finally obtain a volumetric segmentation. In addition, we explore how super-resolution images ($2\sim5$ times beyond the physical CT imaging), generated from a proposed stacked generative adversarial network, can aid the WSSS performance. We employ the DeepLesion dataset, a comprehensive CT-image lesion dataset of $32,735$ PACS-bookmarked findings, which include lesions, tumors, and lymph nodes of varying sizes, categories, body regions and surrounding contexts. These are drawn from $10,594$ studies of $4,459$ patients. We also validate on a lymph-node dataset, where 3D ground truth masks are available for all images. For the DeepLesion dataset, we report mean Dice coefficients of 93\% on RECIST-slices and $76\%$ in 3D lesion volumes. We further validate using a subjective user study, where an experienced radiologist accepted our WSSS-generated lesion segmentation results with a high probability of 92.4\%. 


==> sections/conclusion.tex <==
%! TEX root=../main.tex

In this paper, we present a simple yet surprisingly effective weakly supervised deep segmentation approach on turning massive amounts of RECIST based lesion diameter measurements (retrospectively stored in hospitals' digital repositories) to full 3D lesion volume segmentation and measurements. Our proposed self-paced CNN models can learn and propagate lesion segmentation from RECIST-measured CT slices into 3D lesion volumes. The radiologist's ``zooming'' factor when depicting the lesion diameters on CT images is implemented via our proposed stacked GAN models for image denoising and super-resolution. Importantly, our approach does not require pre-existing RECIST measurements on processing new cases of lesion segmentation.

Our method is fully automatic and learned from a large quantity of ``partially-labeled'' clinical annotations. The lesion segmentation results are validated through both quantitative evaluation (e.g., 93\% mean DICE on RECIST-slices and 76\% for lesion volume segmentation) and subjective user studies. 3D lesion segmentation also produces more accurate estimation on calculating the lesion follow-up volume changes than the RECIST criteria. Our work is potentially of high importance on automated, large-scale tumor volume measurement/management in the domain of precision quantitative radiology imaging.


==> sections/conclusion_Le.tex <==
%! TEX root=../main.tex

We present a simple yet surprisingly effective weakly supervised deep segmentation approach on turning massive amounts of RECIST-based lesion diameter measurements (retrospectively stored in hospitals' digital repositories) to full 3D lesion volume segmentation and measurements. The radiologist's \textit{zooming} factor when depicting the lesion diameters on CT images is emulated via our proposed stacked GAN models for image denoising and super-resolution. Importantly, our approach does not require pre-existing RECIST measurements on processing new cases. % of lesion segmentation.

Our method is fully automatic and learned from a large quantity of \textit{partially-labeled} clinical annotations. The lesion segmentation results are validated through both quantitative evaluation (e.g., $93\%$ mean DICE on RECIST-slices and $76\%$ for 3D lesion volume segmentation) and subjective user studies. We demonstrate that our self-paced learning improves performance over state-of-the-art CNNs. Moreover, we demonstrate how leveraging the weakly supervised, but large-scale data, allows us to outperform fully-supervised approaches that can only be trained on subsets where full masks are available. Our 3D lesion segmentation also produces more accurate estimations of lesion volume changes than the RECIST criteria. Our work is potentially of high importance for automated and large-scale tumor volume measurement/management in the domain of precision quantitative radiology imaging.


==> sections/experiments.tex <==
%!TEX root=../main.tex

%-------------------------------------------------------------------------
%\subsection{Experimental Set Up} \label{sec:exp-sets}
\textbf{Datasets:} The Deep-Lesion dataset \cite{yan_2017_deep-lesion} is composed of 32,735 bookmarked CT lesion instances (with RECIST measurements) from 10,594 studies of 4,459 patients. Lesions has been categorized into \textcolor{red}{8} subtypes by different body sections of lung, mediastinum, liver, soft-tissue, abdomen, kidney, pelvis and bone. To facilitate the quantitative evaluation, we have segmented 1,000 testing lesion RECIST-slices \textcolor{red}{manually}. Out of 1000, 200 lesions ($\sim$3,500 annotated slices) are fully segmented in 3D as well. Furthermore, we employ the lymph node (LN) dataset\footnote{\url{https://wiki.cancerimagingarchive.net/display/Public/CT+Lymph+Nodes}} \cite{roth_2014_lymphnode,Seff20142D}, which consists of 389 mediastinal and 595 abdominal LNs from 176 CT scans with pixel-wise annotations. Enlarged lymph node is a subtype lesion and its segmentation task is quite challenge even with fully supervised learning \cite{n_isabella_miccai2016_lymphnode}. The fully pixel-wise annotated LN dataset can be used to evaluate our weakly supervised lesion segmentation method, by comparing towards the fully supervised approach \cite{n_isabella_miccai2016_lymphnode}. %LN may share similar appearances with abdomen lesions and soft-tissue lesions. %We also study a smaller dataset, the Lymph-Node \cite{roth_2014_lymphnode} \footnote{\url{https://wiki.cancerimagingarchive.net/display/Public/CT+Lymph+Nodes}}, which have been fully annotated in pixel-wise accuracy for enlarged lymph-node in 176 CT volumes. As a subtype of soft-tissue lesion, lymph nodes shares {\textbf{similar visual appearance}} with Deep-Lesions. Working on lymph node segmentation helps us to understand the proposed WSSS method in comprehensive.

{\bf Pre-processing:} The LN annotation mask can be converted into RECIST diameters via regional process measuring the major/minor axes after localizing the 5 successive axial slice nearest to the largest LN cross-section. For robustness, up to 20\% random noises in length are injected for the diameter measurements to mimic the uncertainty of manual annotation by radiologists. Based on the location of RECIST bookmarks, CT sub-volumes are cropped at two times of the lesions' longest diameters so that sufficient background spatial contexts are preserved. Each lesion CT volume is then intensity-windowed properly using the CT windowing meta-information in \cite{yan_2017_deep-lesion}. LN dataset is separated at the patient level, using the split of 80\%/20\% for training and testing respectively. For Deep-Lesion dataset \cite{yan_2017_deep-lesion}, we use 28,000 lesion volumes for training and the rest for testing.

Mean Dice Similarity Coefficient (mDICE), {\small $DICE=2TP/(2TP+FP+FN)$} and the pixel-wise calculated Precision and Recall scores are used to evaluate the quantitative segmentation accuracy. We also employ the metrics of Volume Similarity (VS) {\small $VS=1-(FN-FP)/(2TP+FP+FN)$} and Averaged Hausdorff Distance (AVD) to better capture and evaluate the small but vital changes near object boundaries \cite{t_abdel_bmc15_metrics}.

%Ellipse fitting can be used to approximate the initial foreground lesion segmentation on the RECIST slice so that (weak) supervision is applicable during model training. As tested on Lymph-Node and annotated images in Deep-Lesion, the measuring score of weak supervision is of strong correlation with score from manual ground truth. With strong mDICE, the weak mDICE is of 0.86 and 0.98 Pearson correlation for Deep-Lesion and Lymph-Node in respective. Weak supervision enables model evaluation when we process new lesion data from wild.

Our baseline CNN model is Holistically-Nested Network (HNN), originally proposed for natural image edge detection \cite{s_xie_iccv15_hed}, has been adapted successfully for several medical image applications of lymph node \cite{n_isabella_miccai2016_lymphnode} and pancreas segmentation \cite{j_cai_miccai17_pancreas,r_holger_arxiv16_pancreas}. HNN works slightly better than U-net \cite{ronneberger_2015_unet} as evaluated in \cite{r_holger_arxiv16_pancreas}. In all experiments, CNN training is implemented in Tensorflow with Adam Optimizer and initialized from the pre-trained ImageNet model \cite{s_xie_iccv15_hed}. Learning rate is set as {\small $5\times10^{-5}$} and dropped to {\small $1\times10^{-5}$} when the model training-validation plot plateaus.

\input{data/result_train_mask_init}

{\bf Label Map Initializations:} Both GrabCut \cite{khoreva_cvpr17_simpledoesit,rother_2004_grabcut} and Densely-connected Conditional Random Field (DCRF) \cite{krah_2012_fully-crf} of different conditions are extensively evaluated for initiating the training label maps from lesion RECIST measurements. A tight bounding box (b-box) of lesion can be obtained from any RECIST with 25\% padding (against the lesion's spatial extent). The central 25\% b-box region is set as foreground and areas out of the b-box as background, leaving the margins as uncertain. This is similar to the setting of b-box$^i$ in \cite{khoreva_cvpr17_simpledoesit}. DCRF takes b-box$^i$ as the unary potentials to conduct inference on lesion segmentation using intensity based pairwise potentials \cite{krah_2012_fully-crf}. We empirically find that DCRF is moderately sensitive to the parameter variations on our dataset. The optimal DCRF performance is reported in Table.\ref{tab:mask-init}. We validate GrabCut on three possible Trimap settings: using b-box$^i$ directly (GrabCut$^i$); setting area outside b-box as background and area inside b-box as foreground (GrabCut); and designating areas outside bbox as background and RECIST as foreground (GrabCut-R) where GrabCut-R works the best. The RECIST is first morphologically dilated to occupy $\sim$20\% area of the b-box (Fig. \ref{fig:Self-Paced}). It is critical to have RECIST axes to roughly clamp the foreground pixels when using GrabCut \cite{khoreva_cvpr17_simpledoesit,rother_2004_grabcut}, which is also be observed by \cite{d_pap_iccv17_extreneclick}. Without necessary pixel clamping, GrabCut may fail to segment lymph nodes since the pixel intensity distribution inside lymph nodes is homogeneous and blurry object-level boundaries are presented.

\input{data/result_2d_convnet}
\input{data/result_ablation_sr}
\input{data/result_lesion_2d_seg}

{\bf CNN Training under Different Levels of Supervision:} Following Sec. \ref{sec:init-mask}, there are three ways of generating initial lesion masks on the RECIST-slice: dilated RECIST, GrabCut-R (processed from dilated RECIST) and the full pixel-wise manual annotation (when available). Using the LN dataset \cite{roth_2014_lymphnode,Seff20142D} with manual ground truth, HNNs trained from  these three initializations of label maps achieve 61\%, 70\%, and 71\% mDICE scores, with increased levels of supervision respectively. No extra segmentation refinement options like adaptive sample mining, or weighted training loss are applied. This observation demonstrates the robustness and effectiveness of using GrabCut-R label map initialization, which only performs slightly worse than the fully annotated pixel-wise masks. On the Deep-Lesion dataset \cite{yan_2017_deep-lesion}, HNN trained on GrabCut-R initialization outperforms the deep model learned from dilated RECIST maps by a margin of 25\% in mDICE (90.6\% versus 64.4\%), quantitatively evaluated on the 1,000 annotated testing RECIST-Slices. GrabCut post-processing further improves the better results from 90.6\% to 91.5\%. To validate the beneficial effectiveness of training CNN using a large quantity of weakly supervised or ``imperfectly-labeled'' object masks (e.g., by GrabCut-R), we have separated the 1,000 annotated testing images into five folds and report the mDICE scores over 5-fold cross-validation using HNN \cite{xie_2015_hnn} and UNet \cite{ronneberger_2015_unet} models under fully supervised model training of 800 images in training folds each round. Fully supervised HNN and UNet report 84\% and 73\% mDICE scores in respective, both significantly lower than 90.6\% achieved by the weakly supervised HNN from GrabCut-R. This confirms the importance of training CNNs from a large-scale ``imperfectly-labeled'' dataset. All the results are described in Table. \ref{tab:2d-convnet}. 

\input{figures/offset}
\input{figures/roc}
\input{./data/result_lesion_3d_seg}

\input{figures/visual_examples}

{\bf 3D Segmentation:} In Fig.\ref{fig:offset}, we show the segmentation results on 2D CT slices that are arranged in the order of voxel-distance with respect to the RECIST-selected slice. GrabCut with 3D RECIST initialization (GrabCut-3DE) produces good segmentation ($\sim$91\%) on the RECIST-slice, but can degrade to 55\% mDICE when the off-slice distance raises to 4. This is mainly because 3D RECIST approximation often is not a robust and accurate estimation across slices so that GrabCut can fail to generate good segmentation using the erratic 3D RECIST initialized {\it trimaps}. On the contrary, HNN CNN trained using RECIST-slice generalizes well with large slice offsets. It still gains $>70$\% of mDICE even when the offset distance ranges to 6. HNN deep model learns the CT image foreground/background intensity distributions and the in-plane spatial contexts for lesion segmentation. The configuration of HNN post-processed by GrabCut reports the best performance. The HNN quantitative segmentation performance on the RECIST slice is 91\% mDICE compare to 74\% when the offset is 3 since CT slices with large offsets are not be seen during the training. HNN is further fine-tuned using CT images with offsets, as shown in the \textbf{For Loop} of Alg.\ref{alg:wsss}. Fig.\ref{fig:pr_curves} presents model improvements from the proposed self-paced learning in precision-recall curves. The final 3D segmentation is reported in Table.\ref{tab:lesion-3d}.

{\bf Ablation Study of Stacked-GAN:} Stacked-GAN networks are first trained from the collection of synthesized natural images \cite{ledig2016photo}. To fine-tune using CT images, We process 28,000 training RECIST slices using the current trained SGAN and select a subset of up to 1,000 slice by subjectively inspecting the CT super-resolution results. The selected CT images are subsequently added in training for the next round of SGAN fine-tuning. This iterative process finishes when few new CT images can be added. When HNN is trained in two input channels of CT and SR images, there are noticeable performance improvements in metrics of precision, AVD, VS, and mDICE (see Table.\ref{tab:Ablation-convnet}). AVD score drops by 15\% from 0.230 to 0.189, implying probably better lesion boundary delineation. Category-wise 2D lesion segmentation results are reported in Table \ref{tab:lesion-2d}. The SGAN assisted HNN (CNN-SR) achieves the best results on all lesion categories at 92\% and GrabCut post-processing (CNN-SR-GC) can improve the mDICE score to 93\%.

\subsection{Subjective Clinical Acceptance Evaluation}

%\begin{figure}[t!]
  %\begin{center}
    %\includegraphics[width=0.7\linewidth]{figures/Visual-Acceptance-v2}
  %\end{center}
  %\caption{\textbf{Visual Acceptance of Automatic Segmentation:} Among 1,000 testing images, 796 automatic segmentations have accepted, and 51 have been rejected by both radiologists. While, there has 153 images that both observers have different opinions.}
  %\label{fig:visual-acceptance}
%\end{figure}

The main motivation and goal of this work are exploring the feasibility of replacing and converting the current 2D diameter based lesion measurements into 3D volumetric scores. It is critical to evaluate the clinicians' subjective feedback on the acceptance rates of our WSSS produced lesion segmentation outcomes. The survey on the acceptance rate of automatic segmentation outcomes is conducted by two board-certificated radiologists. 

%% %% 1) The 1,000 testing RECIST-measured lesion CT images (overlaid with manual or automatic segmentation masks) are randomly displayed to radiologists to judge whether to accept the segmentation or not. For WSSS segmentation, radiologists are agreed on accepting 796 segmentation and rejecting 51, while they conflict with each other on 153 images. The acceptance rates of manual segmentation are 97.9\% and 93\%, and 90.1\% and 84.5\% on WSSS segmentation for two radiologists, respectively. 
1) The 1,000 testing RECIST-measured lesion CT images (overlaid with manual or automatic segmentation masks) are randomly displayed to radiologists to judge whether to accept the segmentation or not. For WSSS segmentation, radiologists are agreed on accepting 870 segmentation and rejecting 45, while they conflict with each other on 85 images. The acceptance rates of manual segmentation are 97.9\% and 98.7\%, and 90.1\% and 92.4\% on WSSS segmentation for two radiologists, respectively. 

2) We show both manual and WSSS computed lesion segmentation results simultaneously in shuffled orders to radiologists and let them pick the more preferable result (i,e., human judges do not know which segmentation is the manual ``ground truth''). Consequently, radiologist-A picks 63 ``WSSS-over-manual'' segmentation cases, designate another 619 instances as ``inseparable'' segmentation qualities and marks the left 318 as ``manual-over-WSSS''. The three-class splits for radiologist-B are 72-645-269. 

3) 22 pairs of lesion volumes with follow-ups are selected from our testing dataset. They are used to evaluate the volume changes at two time points via the means of manual segmentation, RECIST measurements, or the proposed WSSS segmentation. For RECIST, lesion volume is estimated by ellipsoid volume as $V = \pi (length \times width^2) / 6$ where $length$ and $width$ present the long and short axes in respective. In Fig.\ref{fig:volume-change}, the volume change plots against the follow-up cases are illustrated. Manual and computerized segmentation results correlate well (the slope of 0.9), whereas the ellipsoid RECIST estimations tend to report smaller-than-actual volume changes (the slope of 0.3).
\begin{figure}[t!]
\begin{center}
  \includegraphics[width=.76\linewidth]{figures/Measure/follow-ups}
\end{center}
\vspace{-4mm}
\caption{{\bf Comparison in Measuring Volume Changes} using manual segmentation, WSSS segmentation and RECIST.}
\label{fig:volume-change}
\end{figure}

%% %% \subsection{Tables}
%% %% \input{./data/lymphnode_recist2mask}
%% %% \input{./data/result_train_mask_init}
%% %% \input{./data/recist_to_mask_init}
%% %%
%% %% \input{./data/hnn_lesion}
%% %% \input{./data/hnn_lesion-sr}
%% %% \input{./data/hnn_lesion_volume}
%% %% \input{./data/hnn_lesion_category}
%% %%
%% %% \input{./data/hnn_lymphnode_mca-3d}
%% %% \input{./data/hnn_lymphnode_mca_train}
%% %% \input{./data/hnn_lymphnode_mca_mask-init}
%% %%
%% %% \input{./data/hnn_lymphnode_train}
%% %% \input{./data/hnn_lymphnode-enhancing_train}
%% %%
%% %% \input{./data/full_weak_metric_correlation}


==> sections/experiments_Jim_single_radiologist.tex <==
%!TEX root=../main.tex

%-------------------------------------------------------------------------
%\subsection{Experimental Set Up} \label{sec:exp-sets}
\textbf{Datasets:} The DeepLesion dataset \cite{yan_2017_deep-lesion} is composed of $32,735$ bookmarked CT lesion instances (with RECIST measurements) from $10,594$ studies of $4,459$ patients. Lesions have been categorized into the $8$ subtypes of lung, mediastinum, liver, soft-tissue, abdomen, kidney, pelvis, and bone. To facilitate quantitative evaluation, we segmented $1,000$ testing lesion RECIST-slices manually. Out of these $1000$, $200$ lesions ($\sim3,500$ annotated slices) are fully segmented in 3D as well. Additionally, we also employ the lymph node (LN) dataset\footnote{\url{https://wiki.cancerimagingarchive.net/display/Public/CT+Lymph+Nodes}} \cite{roth_2014_lymphnode,Seff20142D}, which consists of $389$ mediastinal and $595$ abdominal LNs from $176$ CT scans with complete pixel-wise annotations. Enlarged LNs are a lesion subtype and producing accurate segmentations is quite challenging even with fully supervised learning \cite{n_isabella_miccai2016_lymphnode}. Importantly, the fully annotated LN dataset can be used to evaluate our WSSS method against an upper performance limit, by comparing results with a fully supervised approach \cite{n_isabella_miccai2016_lymphnode}. %LN may share similar appearances with abdomen lesions and soft-tissue lesions. %We also study a smaller dataset, the Lymph-Node \cite{roth_2014_lymphnode} \footnote{\url{https://wiki.cancerimagingarchive.net/display/Public/CT+Lymph+Nodes}}, which have been fully annotated in pixel-wise accuracy for enlarged lymph-node in 176 CT volumes. As a subtype of soft-tissue lesion, lymph nodes shares {\textbf{similar visual appearance}} with Deep-Lesions. Working on lymph node segmentation helps us to understand the proposed WSSS method in comprehensive.

{\bf Pre-processing:} For the LN dataset, annotation masks are converted into RECIST diameters by measuring the major/minor axes after localizing the $5$ successive axial slices nearest to the largest LN cross-section. For robustness, up to $20\%$ random noise is injected in the RECIST diameter lengths to mimic the uncertainty of manual annotation by radiologists. For both datasets, based on the location of RECIST bookmarks, CT ROIs are cropped at two times the extent of the lesion's longest diameters so that sufficient visual context is preserved. The dynamic range of each lesion ROI is then intensity-windowed properly using the CT windowing meta-information in \cite{yan_2017_deep-lesion}. The LN dataset is separated at the patient level, using the split of $80\%$ and $20\%$ for training and testing, respectively. For the DeepLesion dataset \cite{yan_2017_deep-lesion}, we use $28,000$ lesion volumes for training and the rest for testing.

{\bf Evaluation:} The mean dice similarity coefficient (mDICE), {\small $DICE=2TP/(2TP+FP+FN)$} and the pixel-wise precision and recall scores are used to evaluate the quantitative segmentation accuracy. We measure volumetric similarity (VS) {\small $VS=1-(FN-FP)/(2TP+FP+FN)$} and averaged Hausdorff distance (AVD) to better capture and evaluate the small but vital changes near object boundaries \cite{t_abdel_bmc15_metrics}.

%Ellipse fitting can be used to approximate the initial foreground lesion segmentation on the RECIST slice so that (weak) supervision is applicable during model training. As tested on Lymph-Node and annotated images in Deep-Lesion, the measuring score of weak supervision is of strong correlation with score from manual ground truth. With strong mDICE, the weak mDICE is of 0.86 and 0.98 Pearson correlation for Deep-Lesion and Lymph-Node in respective. Weak supervision enables model evaluation when we process new lesion data from wild.

Our baseline CNN model is the holistically-nested network (HNN), originally proposed for natural image edge detection \cite{s_xie_iccv15_hed}, which has been adapted successfully for lymph node \cite{n_isabella_miccai2016_lymphnode}, pancreas \cite{j_cai_miccai17_pancreas,r_holger_arxiv16_pancreas}, and lung segmentation \cite{Harrison_2017}. In all experiments, CNN training is implemented in Tensorflow with Adam Optimizer and initialized from the pre-trained ImageNet model \cite{s_xie_iccv15_hed}. The learning rate is set as {\small $5\times10^{-5}$} and it drops to {\small $1\times10^{-5}$} when the model training-validation plot plateaus.

\input{data/result_train_mask_init}

{\bf Label Map Initializations:} Both GrabCut \cite{khoreva_cvpr17_simpledoesit,rother_2004_grabcut} and densely-connected conditional random fields (DCRF) \cite{krah_2012_fully-crf} are extensively evaluated for initializing training label maps from RECIST diameters. We test two alternatives to the \textit{trimap} approach explained in Sec.~\ref{sec:init-mask}, which we denote GrabCut-R. Both alternatives are based on a tight bounding box (bbox), which matches the extent of the lesion RECIST marks with $25\%$ padding (against the lesion's spatial extent). The first alternative (GrabCut), sets the area outside bbox as background and area inside bbox as probable foreground. The second alternative (GrabCut$^i$) sets the central $20\%$ bbox region as foreground, regions outside the bbox as background, and the rest as uncertain. This is similar to the setting of bbox$^i$ in \cite{khoreva_cvpr17_simpledoesit}. We also test DCRF, using bbox$^i$ as the unary potentials and intensities to compute pairwise potentials \cite{krah_2012_fully-crf}. We empirically found that DCRF is moderately sensitive to parameter variations. The optimal DCRF performance is reported in Table~\ref{tab:mask-init}. Finally, we also report results when we directly use the RECIST diameters, but dilated to $20\%$ of bbox area, which unsurprisingly produces the best precision, but at the cost of very low recall. However, as can be seen in the table, GrabCut-R significantly outperforms all alternatives, demonstrating the validity of our mask initialization process. 

\input{data/result_2d_convnet}
%We also observe that it is critical to have RECIST axes to roughly clamp the foreground pixels when using GrabCut \cite{khoreva_cvpr17_simpledoesit,rother_2004_grabcut}, which is also be observed by \cite{d_pap_iccv17_extreneclick}. Without necessary pixel clamping, GrabCut may fail to segment lymph nodes since the pixel intensity distribution inside lymph nodes is homogeneous and blurry object-level boundaries are presented.

{\bf CNN Training under Different Levels of Supervision:} Following Sec. \ref{sec:init-mask}, there are three ways of generating initial lesion masks on the RECIST-slice: using the \textit{trimap} from the dilated RECIST (ignoring uncertain regions in training), GrabCut-R (processed from the \textit{trimap}) and the full pixel-wise manual annotation (when available). Using the LN dataset \cite{roth_2014_lymphnode,Seff20142D} with manual ground truth, HNNs trained from  these three initializations of label maps achieve 61\%, 70\%, and 71\% mDICE scores, with increased levels of supervision respectively. No extra segmentation refinement options like adaptive sample mining, or weighted training loss are applied. This observation demonstrates the robustness and effectiveness of using GrabCut-R label map initialization, which only performs slightly worse than the fully annotated pixel-wise masks. On the DeepLesion~\cite{yan_2017_deep-lesion} testset of $1,000$ annotated testing RECIST-slices, HNN trained on GrabCut-R initialization outperforms the deep model learned from dilated RECIST maps by a margin of 25\% in mDICE (90.6\% versus 64.4\%). GrabCut post-processing further improves the results from 90.6\% to 91.5\%. We also aim to demonstrate that our WSSS approach, trained on a large quantity of weakly supervised or ``imperfectly-labeled'' object masks, can outperform fully-supervised models trained on less data. To do this, we separated the $1,000$ annotated testing images into five folds and report the mDICE scores over 5-fold cross-validation using fully-supervised HNN~\cite{xie_2015_hnn} and UNet~\cite{ronneberger_2015_unet} models. Impressively, the $90.6\%$ dice score of WSSS considerably outperforms the fully supervised HNN and UNet mDICE scores of $84\%$ and $73\%$, respectively. This demonstrates the importance of training CNNs from a large-scale ``imperfectly-labeled'' dataset. All the results are described in Table~\ref{tab:2d-convnet}. 

\input{figures/offset}
\input{figures/roc}
\input{data/result_ablation_sr}
\input{data/result_lesion_2d_seg}

{\bf 3D Segmentation:} In Fig.~\ref{fig:offset}, we show the segmentation results on 2D CT slices arranged in the order of voxel-distance with respect to the RECIST-selected slice. GrabCut with 3D RECIST initialization (GrabCut-3DE) produces good segmentations ($\sim$91\%) on the RECIST-slice, but can degrade to 55\% mDICE when the off-slice distance raises to 4. This is mainly because 3D RECIST approximation often is not a robust and accurate estimation across slices. %using the unreliable \textit{trimaps} initialized from the 3D RECIST estimation. 
In contrast, the HNN trained using RECIST-slices generalizes well with large slice offsets. It still gains $>70$\% of mDICE even when the offset distance range as high as $6$. However, performance is further improved at higher slice offsets when using self-paced learning with $3$ axial slices, \ie{}, WSSS (mid), and even further when using the full self-paced learning with $5$ axial slices, \ie{}, WSSS.  These results demonstrate the value of using our self-paced learning approach to generalize beyond 2D RECIST slices into full 3D segmentations. Fig.~\ref{fig:pr_curves} further demonstrates the model improvements from self-paced learning using precision-recall curves. Unsurprisingly, the WSSS schemes do not provide much improvement on the 2D RECIST slices; however, significant improvements are garnered when considering the full 3D segmentations, again demonstrating the benefits of WSSS to achieve clinically useful volumetric lesion segmentations. The final 3D segmentation results are tabulated in Table~\ref{tab:lesion-3d}.

\input{./data/result_lesion_3d_seg}
\input{figures/visual_examples_single_radiologist}

{\bf Ablation Study of Stacked-GAN:} When we train the HNN using two input channels of original CT and super resolution (SR) images, there are significant improvements in the precision, AVD, VS, and mDICE metrics (see Table.\ref{tab:Ablation-convnet}). In particular, the AVD scores drop by $15\%$ from $0.230$ to $0.189$, likely implying better lesion boundary delineation. Category-wise 2D lesion segmentation results are reported in Table \ref{tab:lesion-2d}. The SGAN assisted HNN (HNN-SR) improves over standard HNN, and, with GrabCut post-processing, the best result of $93\%$ mDICE score is achieved.

\subsection{Subjective Clinical Acceptance Evaluation}
The main motivation and goal of this work is exploring the feasibility of replacing and converting the current 2D RECIST diameter based lesion measurements into 3D volumetric scores. Consequently, it is critical to evaluate clinician's subjective feedback on the acceptance rates of our WSSS produced lesion segmentations. We measure the acceptance rates of a US board-certificated radiologist with over 25 years of clinical practice experience under two different scenarios.

1) The $1,000$ testing RECIST-measured lesion CT images (overlaid with manual or automatic segmentation masks) are randomly displayed to the experienced radiologist to judge whether to accept the segmentation or not. The acceptance rate for WSSS segmentations is $92.4\%$, which is close to the $97.9\%$ acceptance rate of the manually segmented masks (which were performed by a radiology resident). Examples of accepted and rejected automatic segmentations are displayed in Fig.~\ref{fig:visual-example}.

2) We show both manual and WSSS computed lesion segmentation results simultaneously in shuffled orders to the radiologist and let him pick the more preferable result (\ie{}, the human judge does not know which segmentation mask is the manual \textit{ground truth}). Consequently, the radiologist picks $72$ \textit{WSSS-over-manual} segmentation cases, designates another $645$ instances as \textit{inseparable} in segmentation quality, and marks the remaining $269$ as \textit{manual-over-WSSS}. 

\begin{figure}[t!]
	\begin{center}
		\includegraphics[width=.76\linewidth]{figures/Measure/follow-ups}
	\end{center}
	\vspace{-4mm}
	\caption{{\bf Volume Measurements:} Volume changes measured using manual segmentations are graphed vs. WSSS and RECIST-based segmentation. Lines of best fit are also rendered.}
	\label{fig:volume-change}
\end{figure}

Finally, we also measure how well the WSSS method can track lesion changes over time. Toward this end, $22$ pairs of lesion volumes with follow-ups are selected from our test dataset. They are used to evaluate the volume changes at two time points via the means of manual segmentation, RECIST measurements, or the proposed WSSS segmentation. For RECIST, the lesion volume is estimated by ellipsoid volume as $V = \pi (length \times width^2) / 6$ where $length$ and $width$ represent the long and short axes, respectively. In Fig.~\ref{fig:volume-change}, the volume change plots against the follow-up cases are illustrated. Manual and computerized segmentation results correlate well (with a slope of $0.9$), whereas the ellipsoid RECIST estimations tend to report smaller-than-actual volume changes (with a slope of $0.3$).


==> sections/experiments_jim.tex <==
%!TEX root=../main.tex

%-------------------------------------------------------------------------
%\subsection{Experimental Set Up} \label{sec:exp-sets}
\textbf{Datasets:} The Deep-Lesion dataset \cite{yan_2017_deep-lesion} is composed of 32,735 bookmarked CT lesion instances (with RECIST measurements) from 10,594 studies of 4,459 patients. Lesions has been categorized into \textcolor{red}{8} subtypes by different body sections of lung, mediastinum, liver, soft-tissue, abdomen, kidney, pelvis and bone. To facilitate the quantitative evaluation, we have segmented 1,000 testing lesion RECIST-slices \textcolor{red}{manually}. Out of 1000, 200 lesions ($\sim$3,500 annotated slices) are fully segmented in 3D as well. Furthermore, we employ the lymph node (LN) dataset\footnote{\url{https://wiki.cancerimagingarchive.net/display/Public/CT+Lymph+Nodes}} \cite{roth_2014_lymphnode,Seff20142D}, which consists of 389 mediastinal and 595 abdominal LNs from 176 CT scans with pixel-wise annotations. Enlarged lymph node is a subtype lesion and its segmentation task is quite challenge even with fully supervised learning \cite{n_isabella_miccai2016_lymphnode}. The fully pixel-wise annotated LN dataset can be used to evaluate our weakly supervised lesion segmentation method, by comparing towards the fully supervised approach \cite{n_isabella_miccai2016_lymphnode}. %LN may share similar appearances with abdomen lesions and soft-tissue lesions. %We also study a smaller dataset, the Lymph-Node \cite{roth_2014_lymphnode} \footnote{\url{https://wiki.cancerimagingarchive.net/display/Public/CT+Lymph+Nodes}}, which have been fully annotated in pixel-wise accuracy for enlarged lymph-node in 176 CT volumes. As a subtype of soft-tissue lesion, lymph nodes shares {\textbf{similar visual appearance}} with Deep-Lesions. Working on lymph node segmentation helps us to understand the proposed WSSS method in comprehensive.

{\bf Pre-processing:} The LN annotation mask can be converted into RECIST diameters via regional process measuring the major/minor axes after localizing the 5 successive axial slice nearest to the largest LN cross-section. For robustness, up to 20\% random noises in length are injected for the diameter measurements to mimic the uncertainty of manual annotation by radiologists. Based on the location of RECIST bookmarks, CT sub-volumes are cropped at two times of the lesions' longest diameters so that sufficient background spatial contexts are preserved. Each lesion CT volume is then intensity-windowed properly using the CT windowing meta-information in \cite{yan_2017_deep-lesion}. LN dataset is separated at the patient level, using the split of 80\%/20\% for training and testing respectively. For Deep-Lesion dataset \cite{yan_2017_deep-lesion}, we use 28,000 lesion volumes for training and the rest for testing.

Mean Dice Similarity Coefficient (mDICE), {\small $DICE=2TP/(2TP+FP+FN)$} and the pixel-wise calculated Precision and Recall scores are used to evaluate the quantitative segmentation accuracy. We also employ the metrics of Volume Similarity (VS) {\small $VS=1-(FN-FP)/(2TP+FP+FN)$} and Averaged Hausdorff Distance (AVD) to better capture and evaluate the small but vital changes near object boundaries \cite{t_abdel_bmc15_metrics}.

%Ellipse fitting can be used to approximate the initial foreground lesion segmentation on the RECIST slice so that (weak) supervision is applicable during model training. As tested on Lymph-Node and annotated images in Deep-Lesion, the measuring score of weak supervision is of strong correlation with score from manual ground truth. With strong mDICE, the weak mDICE is of 0.86 and 0.98 Pearson correlation for Deep-Lesion and Lymph-Node in respective. Weak supervision enables model evaluation when we process new lesion data from wild.

Our baseline CNN model is Holistically-Nested Network (HNN), originally proposed for natural image edge detection \cite{s_xie_iccv15_hed}, has been adapted successfully for several medical image applications of lymph node \cite{n_isabella_miccai2016_lymphnode} and pancreas segmentation \cite{j_cai_miccai17_pancreas,r_holger_arxiv16_pancreas}. HNN works slightly better than U-net \cite{ronneberger_2015_unet} as evaluated in \cite{r_holger_arxiv16_pancreas}. In all experiments, CNN training is implemented in Tensorflow with Adam Optimizer and initialized from the pre-trained ImageNet model \cite{s_xie_iccv15_hed}. Learning rate is set as {\small $5\times10^{-5}$} and dropped to {\small $1\times10^{-5}$} when the model training-validation plot plateaus.

\input{data/result_train_mask_init}

{\bf Label Map Initializations:} Both GrabCut \cite{khoreva_cvpr17_simpledoesit,rother_2004_grabcut} and Densely-connected Conditional Random Field (DCRF) \cite{krah_2012_fully-crf} of different conditions are extensively evaluated for initiating the training label maps from lesion RECIST measurements. A tight bounding box (b-box) of lesion can be obtained from any RECIST with 25\% padding (against the lesion's spatial extent). The central 25\% b-box region is set as foreground and areas out of the b-box as background, leaving the margins as uncertain. This is similar to the setting of b-box$^i$ in \cite{khoreva_cvpr17_simpledoesit}. DCRF takes b-box$^i$ as the unary potentials to conduct inference on lesion segmentation using intensity based pairwise potentials \cite{krah_2012_fully-crf}. We empirically find that DCRF is moderately sensitive to the parameter variations on our dataset. The optimal DCRF performance is reported in Table.\ref{tab:mask-init}. We validate GrabCut on three possible Trimap settings: using b-box$^i$ directly (GrabCut$^i$); setting area outside b-box as background and area inside b-box as foreground (GrabCut); and designating areas outside bbox as background and RECIST as foreground (GrabCut-R) where GrabCut-R works the best. The RECIST is first morphologically dilated to occupy $\sim$20\% area of the b-box (Fig. \ref{fig:Self-Paced}). It is critical to have RECIST axes to roughly clamp the foreground pixels when using GrabCut \cite{khoreva_cvpr17_simpledoesit,rother_2004_grabcut}, which is also be observed by \cite{d_pap_iccv17_extreneclick}. Without necessary pixel clamping, GrabCut may fail to segment lymph nodes since the pixel intensity distribution inside lymph nodes is homogeneous and blurry object-level boundaries are presented.

\input{data/result_2d_convnet}
\input{data/result_ablation_sr}
\input{data/result_lesion_2d_seg}

{\bf CNN Training under Different Levels of Supervision:} Following Sec. \ref{sec:init-mask}, there are three ways of generating initial lesion masks on the RECIST-slice: dilated RECIST, GrabCut-R (processed from dilated RECIST) and the full pixel-wise manual annotation (when available). Using the LN dataset \cite{roth_2014_lymphnode,Seff20142D} with manual ground truth, HNNs trained from  these three initializations of label maps achieve 61\%, 70\%, and 71\% mDICE scores, with increased levels of supervision respectively. No extra segmentation refinement options like adaptive sample mining, or weighted training loss are applied. This observation demonstrates the robustness and effectiveness of using GrabCut-R label map initialization, which only performs slightly worse than the fully annotated pixel-wise masks. On the Deep-Lesion dataset \cite{yan_2017_deep-lesion}, HNN trained on GrabCut-R initialization outperforms the deep model learned from dilated RECIST maps by a margin of 25\% in mDICE (90.6\% versus 64.4\%), quantitatively evaluated on the 1,000 annotated testing RECIST-Slices. GrabCut post-processing further improves the better results from 90.6\% to 91.5\%. To validate the beneficial effectiveness of training CNN using a large quantity of weakly supervised or ``imperfectly-labeled'' object masks (e.g., by GrabCut-R), we have separated the 1,000 annotated testing images into five folds and report the mDICE scores over 5-fold cross-validation using HNN \cite{xie_2015_hnn} and UNet \cite{ronneberger_2015_unet} models under fully supervised model training of 800 images in training folds each round. Fully supervised HNN and UNet report 84\% and 73\% mDICE scores in respective, both significantly lower than 90.6\% achieved by the weakly supervised HNN from GrabCut-R. This confirms the importance of training CNNs from a large-scale ``imperfectly-labeled'' dataset. All the results are described in Table. \ref{tab:2d-convnet}. 

\input{figures/offset}
\input{figures/roc}
\input{./data/result_lesion_3d_seg}

\input{figures/visual_examples}

{\bf 3D Segmentation:} In Fig.\ref{fig:offset}, we show the segmentation results on 2D CT slices that are arranged in the order of voxel-distance with respect to the RECIST-selected slice. GrabCut with 3D RECIST initialization (GrabCut-3DE) produces good segmentation ($\sim$91\%) on the RECIST-slice, but can degrade to 55\% mDICE when the off-slice distance raises to 4. This is mainly because 3D RECIST approximation often is not a robust and accurate estimation across slices so that GrabCut can fail to generate good segmentation using the erratic 3D RECIST initialized {\it trimaps}. On the contrary, HNN CNN trained using RECIST-slice generalizes well with large slice offsets. It still gains $>70$\% of mDICE even when the offset distance ranges to 6. HNN deep model learns the CT image foreground/background intensity distributions and the in-plane spatial contexts for lesion segmentation. The configuration of HNN post-processed by GrabCut reports the best performance. The HNN quantitative segmentation performance on the RECIST slice is 91\% mDICE compare to 74\% when the offset is 3 since CT slices with large offsets are not be seen during the training. HNN is further fine-tuned using CT images with offsets, as shown in the \textbf{For Loop} of Alg.\ref{alg:wsss}. Fig.\ref{fig:pr_curves} presents model improvements from the proposed self-paced learning in precision-recall curves. The final 3D segmentation is reported in Table.\ref{tab:lesion-3d}.

{\bf Ablation Study of Stacked-GAN:} Stacked-GAN networks are first trained from the collection of synthesized natural images \cite{ledig2016photo}. To fine-tune using CT images, We process 28,000 training RECIST slices using the current trained SGAN and select a subset of up to 1,000 slice by subjectively inspecting the CT super-resolution results. The selected CT images are subsequently added in training for the next round of SGAN fine-tuning. This iterative process finishes when few new CT images can be added. When HNN is trained in two input channels of CT and SR images, there are noticeable performance improvements in metrics of precision, AVD, VS, and mDICE (see Table.\ref{tab:Ablation-convnet}). AVD score drops by 15\% from 0.230 to 0.189, implying probably better lesion boundary delineation. Category-wise 2D lesion segmentation results are reported in Table \ref{tab:lesion-2d}. The SGAN assisted HNN (CNN-SR) achieves the best results on all lesion categories at 92\% and GrabCut post-processing (CNN-SR-GC) can improve the mDICE score to 93\%.

\subsection{Subjective Clinical Acceptance Evaluation}

%\begin{figure}[t!]
  %\begin{center}
    %\includegraphics[width=0.7\linewidth]{figures/Visual-Acceptance-v2}
  %\end{center}
  %\caption{\textbf{Visual Acceptance of Automatic Segmentation:} Among 1,000 testing images, 796 automatic segmentations have accepted, and 51 have been rejected by both radiologists. While, there has 153 images that both observers have different opinions.}
  %\label{fig:visual-acceptance}
%\end{figure}

The main motivation and goal of this work are exploring the feasibility of replacing and converting the current 2D diameter based lesion measurements into 3D volumetric scores. It is critical to evaluate the clinicians' subjective feedback on the acceptance rates of our WSSS produced lesion segmentation outcomes. The survey on the acceptance rate of automatic segmentation outcomes is conducted by a board-certificated radiologists. 

%% %% 1) The 1,000 testing RECIST-measured lesion CT images (overlaid with manual or automatic segmentation masks) are randomly displayed to radiologists to judge whether to accept the segmentation or not. For WSSS segmentation, radiologists are agreed on accepting 796 segmentation and rejecting 51, while they conflict with each other on 153 images. The acceptance rates of manual segmentation are 97.9\% and 93\%, and 90.1\% and 84.5\% on WSSS segmentation for two radiologists, respectively. 
1) The 1,000 testing RECIST-measured lesion CT images (overlaid with manual or automatic segmentation masks) are randomly displayed to the radiologists to judg whether to accept the segmentation or not. For WSSS segmentation, the radiologist accepted 924 segmentation and rejected the rest 76 cases. 

2) We show both manual and WSSS computed lesion segmentation results simultaneously in shuffled orders to radiologists and let them pick the more preferable result (i,e., human judges do not know which segmentation is the manual ``ground truth''). Consequently, the radiologist picks 72 ``WSSS-over-manual'' segmentation cases, designate another 645 instances as ``inseparable'' segmentation qualities and marks the left 269 as ``manual-over-WSSS''. 

3) 22 pairs of lesion volumes with follow-ups are selected from our testing dataset. They are used to evaluate the volume changes at two time points via the means of manual segmentation, RECIST measurements, or the proposed WSSS segmentation. For RECIST, lesion volume is estimated by ellipsoid volume as $V = \pi (length \times width^2) / 6$ where $length$ and $width$ present the long and short axes in respective. In Fig.\ref{fig:volume-change}, the volume change plots against the follow-up cases are illustrated. Manual and computerized segmentation results correlate well (the slope of 0.9), whereas the ellipsoid RECIST estimations tend to report smaller-than-actual volume changes (the slope of 0.3).
\begin{figure}[t!]
\begin{center}
  \includegraphics[width=.76\linewidth]{figures/Measure/follow-ups}
\end{center}
\vspace{-4mm}
\caption{{\bf Comparison in Measuring Volume Changes} using manual segmentation, WSSS segmentation and RECIST.}
\label{fig:volume-change}
\end{figure}

%% %% \subsection{Tables}
%% %% \input{./data/lymphnode_recist2mask}
%% %% \input{./data/result_train_mask_init}
%% %% \input{./data/recist_to_mask_init}
%% %%
%% %% \input{./data/hnn_lesion}
%% %% \input{./data/hnn_lesion-sr}
%% %% \input{./data/hnn_lesion_volume}
%% %% \input{./data/hnn_lesion_category}
%% %%
%% %% \input{./data/hnn_lymphnode_mca-3d}
%% %% \input{./data/hnn_lymphnode_mca_train}
%% %% \input{./data/hnn_lymphnode_mca_mask-init}
%% %%
%% %% \input{./data/hnn_lymphnode_train}
%% %% \input{./data/hnn_lymphnode-enhancing_train}
%% %%
%% %% \input{./data/full_weak_metric_correlation}


==> sections/introduction.tex <==
\begin{figure}[t!]
\begin{center}
  \includegraphics[width=\linewidth]{figures/overview_small2.pdf}
\end{center}
\vspace{-4mm}
\caption{Overview of the proposed weakly supervised self-paced segmentation with CNN (Sec.\ref{sec:method}) for 3D lesion segmentation.} 
\label{fig:Self-Paced}
\end{figure}

Assessing lesion or tumor growth rates of multiple time-point scans of the same patient represents one of the most critical problems in imaging-based precision medicine. To track lesion progression using current clinical protocols, radiologists manually conduct this task using response evaluation criteria in solid tumors (RECIST)~\cite{eisenhauer_2009_recist}  in computed tomography (CT) or magnetic resonance imaging (MRI) scans. A radiologist first selects an axial image slice where the lesion has the longest spatial extent, then he or she measures the diameters of the in-plane longest axis and the orthogonal short axis. Fig.~\ref{fig:data-category} provides some visual examples of RECIST marks provided in DeepLesion dataset \cite{yan_2017_deep-lesion}. Typically, the selected RECIST-slice represents the lesion at its maximum cross area. RECIST is often subjective and prone to inconsistency among different observers, especially when selecting the corresponding slices at different time-points where diameters are measured. However, consistency is critical in assessing actual lesion growth rates, which directly impact patient treatment options. On the other hand, if the volumetric lesion measurements between baseline and follow-ups can be accurately computed and compared, this would avoid the subjective selection of RECIST-slices and allow more holistic and accurate quantitative assessment of lesion growth rates. Unfortunately, full volumetric lesion measurements are too labor intensive to obtain. For this reason, RECIST is treated as the default, but imperfect, clinical surrogate of measuring lesion progression. 

Since the clinical adoption of the RECIST criteria, many modern hospitals' picture archiving and communication systems (PACS) and radiology information systems (RIS) have stored tremendous amounts of lesion diameter measurements linked to lesion CT and MRI images. In this paper, we tackle the challenging problem of leveraging existing RECIST diameters to produce fully volumetric lesion segmentation in 3D. Our approach is a weakly supervised semantic segmentation setup, using convolutional neural networks (CNNs) as the core building block. The overall method flow-chart is given in Fig.~\ref{fig:Self-Paced}. DeepLesion database \cite{yan_2017_deep-lesion} that we exploit is composed of a very large number of $32,735$ significant clinical radiology findings (lesions, tumors, lymph nodes, etc) from $10,594$ studies of $4,459$ patients, bookmarked and measured via RECIST diameters by physicians as part of their day-to-day work. The lesion instances are also clustered into eight different anatomical categories as shown in Fig.~\ref{fig:data-category}. Without loss of generality, here we only consider CT lesion images. 

From any input CT image with RECIST-measured diameters, we aim to segment the lesion region on the RECIST-selected image first in a weakly supervised manner, followed by generalizing the process into other successive slices to finally obtain the lesion's full volume segmentation. More specifically, with the bookmarked long and short RECIST diameters, we initialize the segmentation using unsupervised learning methods (\eg{}, GrabCut \cite{rother_2004_grabcut}). Afterwards we employ an iterative segmentation refinement via a supervised deep neural network model \cite{khoreva_cvpr17_simpledoesit}, which can segment the lesion with good accuracy on the RECIST-slice. Importantly, the resulting CNN lesion segmentation model, trained from all training instances of CT RECIST-slices, can capture the lesion image appearance distribution. Thus, the model is  capable of detecting lesion regions from images off the corresponding RECIST-slice. With more slices segmented, more image data can be extracted and used to fine-tune the deep CNN lesion segmentation model. As such, the proposed weakly supervised segmentation model is a self-paced label-map propagation process, from the RECIST-slice to the whole lesion volume. Therefore, we leverage a large amount of retrospective (yet clinically annotated) imaging data to automatically achieve the final 3D lesion volume measurement and segmentation. %, and no extra human annotation efforts are further needed.

To further enhance our WSSS model, we also investigate the role of image enhancement. A large portion of clinically significant findings in DeepLesion are spatially small ($5\sim10$ mm), which often require significant zooming by radiologists to make precise diameter measurements. To emulate this radiological practice, we develop a stacked generative adversarial network (SGAN)~\cite{ledig2016photo} model to perform resolution magnification, noise reduction, contrast enhancement and boundary clearing from the original resolution CT images. We stack two GANs together, where the first reduces the noise from original CT image and the second generates a higher resolution image with enhanced boundaries and high contrast. Because the CT modality can only be imaged at a limited range spatial resolution ($\sim 1$ mm/pixel) and super-resolution CT images (\eg{}, $\sim0.2$ mm/pixel) do not physically exist, we train our SGAN on a large quantity of paired low- and high-quality natural images and use transfer learning to apply the model to CT images.

We evaluate the proposed WSSS segmentation method using all lesion categories~\cite{yan_2017_deep-lesion}. To the best of our knowledge, this is the first work to develop a class-agnostic lesion segmentation approach. For quantitative evaluation, we manually annotated 1,000 RECIST-slices and 200 lesion volumes, where the proposed WSSS achieves mean Dice coefficients of $93\%$ and $76\%$, respectively. To compare WSSS against a fully-supervised approach, we also validate on a lymph node (LN) dataset \cite{roth_2014_lymphnode,Seff20142D}, consisting of $984$ LNs with full pixel-wise annotations. Finally, we also conduct a subjective user study, and demonstrate that radiologist accept the WSSS generated lesion masks with high probability of 92.4\%. %Additionally, we employ the lymph node (LN) dataset \cite{roth_2014_lymphnode,Seff20142D}, consisting of 389 mediastinal and 595 abdominal LNs from 176 CT scans with full pixel-wise annotations \cite{n_isabella_miccai2016_lymphnode}. As one subtype lesion, the task of enlarged lymph node segmentation itself can be very challenge even under the fully supervised setting \cite{n_isabella_miccai2016_lymphnode}. LN may share similar appearances with abdomen lesions and soft-tissue lesions. The pixel-wise annotated Lymph-Node dataset \cite{n_isabella_miccai2016_lymphnode} makes it possible to evaluate our weakly supervised method by comparing it with the fully supervised learning performance.
In summary, we present a weakly supervised semantic segmentation approach for accurate lesion segmentation and volume measurements in the wild, using a comprehensive dataset \cite{yan_2017_deep-lesion}. With no extra human annotation efforts required, we convert tens of thousands of recorded RECIST 2D diameter based measurements in PACS/RIS into accurate 3D lesion volume segmentation assessments. %For the rest of this paper, we discuss related work in Sec.\ref{sec:related-work} and describe our proposed self-paced weakly supervised deep segmentation method in Sec.\ref{sec:method}. The segmentation enhancement by conducting cascaded GAN based image super-resolution is also addressed. The extensive experimental evaluations are given in Sec.\ref{sec:exp}, and finally we conclude our work in Sec.\ref{sec:conclusion}.

\input{figures/data_category}


==> sections/method.tex <==
%!TEX root=../main.tex
\begin{figure*}[t!]
\begin{center}
   \includegraphics[width=0.96\linewidth]{figures/OverView2.pdf}
\end{center}
\caption{Our weakly supervised deep lesion segmentation framework.}
\label{fig:overview}
\end{figure*}

%-------------------------------------------------------------------------
In the DeepLesion dataset \cite{yan_2017_deep-lesion}, manually selected axial CT slices contain RECIST diameters that represent the longest axis and its perpendicular counterpart. Given RECIST diameters as weak supervision, we leverage WSSS principles to learn a deep lesion CNN segmentation model using both 2D slice and 3D volumes with no extra pixel-wise manual annotations. Our pipeline for WSSS contains four major steps: 1) converting RECIST diameters to training masks, 2) learning a 2D CNN lesion appearance model, 3) expanding the 2D model into 3D segmentation, and optionally 4) using SGAN to generate enhanced images as input. 

\subsection{From RECIST to 2D Training Masks} \label{sec:init-mask}
We denote elements in the DeepLesion dataset \cite{yan_2017_deep-lesion} as {\small $D={(V^i,R^i)}$} for {\small $i \in \{1,\ldots,N\}$}, where {\small $N$} is the number of lesions, {\small $V^i$} is the CT region of interest, and {\small $R^i$} is the corresponding RECIST diameters. For notational clarity, we drop the superscript $i$. To create the 2D training data for the WSSS model, the images and label map pairs, {\small $X$ and $Y$}, respectively, must be generated. {\small $X$} is simply the RECIST-slice, \ie{}, the axial slice that contains {\small $R$}. Both GrabCut \cite{rother_2004_grabcut} and densely-connected conditional random fields (DeCRFs) \cite{krah_2012_fully-crf} can be adopted to produce the training mask $Y$. When GrabCut starts with a good quality initial \textit{trimap} (explained below), we observe that it produces better results, which is consistent with the findings in \cite{khoreva_cvpr17_simpledoesit}. 

More specifically, GrabCut is initialized with the image foreground and background regions and produces a segmentation using iterative energy minimization. Good initializations located near the global energy minimum may aid GrabCut's convergence. We use the spatial prior information, provided by {\small $R$}, to compute a high quality initial \textit{trimap} {\small $T$} from {\small $R$}, \ie{}, regions of probable background (PBG), probable foreground (PFG), background (BG), and foreground (FG)~\cite{rother_2004_grabcut}. More specifically, if the lesion bounding box tightly around the RECIST axes is $[w,h]$, a $[2w,2h]$ ROI is cropped from the RECIST-slice. The \textit{trimap} assigns the outer $50\%$ as BG and allocates $10\%$ of the image region, dilated from {\small $R$} as FG. The remaining $40\%$ is divided in half between PFG and PBG based on the distances to FG and BG. Finally, the long/short axes of $R$ roughly clamp the size of GrabCut segmentation, ensuring that the segmentation will not shrink into a small region when the CT image intensity distribution is homogeneous and no clear lesion boundary is presented. Fig.~\ref{fig:overview} visually depicts the mask generation process.

%-------------------------------------------------------------------------
\subsection{CNN Lesion Appearance Model}

Many image classification or segmentation CNN models have been presented in recent works \cite{simonyan_2014_vggnet,he_2016_resnet,huang_2017_densenet,xie_2015_hnn,ronneberger_2015_unet}. Without loss of generality, we use the holistically-nested network (HNN) \cite{xie_2015_hnn} and U-Net \cite{ronneberger_2015_unet} as our baselines, both of which provide state-of-the-art, yet straightforward semantic architectures. We represent our CNN models as a mapping function {\small $\hat{Y} = f(X;\theta)$}, with the goal of optimizing {\small $\theta$} to minimize the differences between the current model outputs {\small $\hat{Y}$} and ground truth training labels {\small $Y$}. Although the Grabcut masks are imperfect, we use them as {\small $Y$} for the next step of CNN model training, expecting that the CNN will generalize well even with considerable label noise. Thus, we aim to minimize
\begin{equation} \label{eq:convnet}
	L(d; \theta) = \frac{1}{N} \sum\limits_{i=1}^{N} \frac{\sum\limits_{m\in Y^i} H (\hat{y}^{(i,m)},y^{(i,m)})}{|Y^i|} \textrm{,}
\end{equation}
where {\small $m$} is the pixel index inside {\small $Y$}, {\small $|Y|$} is the cardinality of {\small $Y$}, and {\small $H(.)$} is the cross-entropy function. %Model parameter {\small $\theta$} is then updated by error backpropagation via SGD.

%-------------------------------------------------------------------------
\subsection{Self-Pacing for Volume Segmentation} \label{sec:3d-wsss}

For obtaining 3D volume segmentations, we follow a similar strategy as with the RECIST slices, except in the 3D case, we must infer $R$ for off-RECIST slices and also incorporate inferences from the CNN model. These two priors are used together for self-paced CNN training.

\textbf{3D RECIST Estimation:} A simple way to generate off-RECIST-slice  {\small $R$} diameters is to take advantage of the fact that RECIST-slice {\small $R$}'s lie on the maximal cross-sectional area of the lesion. The rate of reduction of off-RECIST-slice endpoints is then calculated by their relative distance to the intersection point of the major and minor axes. Estimated 3D RECIST endpoints are then projected from the actual RECIST endpoints by Pythagorean theorem using physical Euclidean distance.

\textbf{Trimap from CNN Output:} Different from Sec.~\ref{sec:init-mask}, \textit{trimap} generation now takes both the CNN output {\small $\hat{Y}$} and the estimated RECIST {\small $\hat{R}$} as inputs: {\small $\hat{T} = trimap(\hat{Y},\hat{R},R)$}. The {\small $\hat{Y}$} is first binarized by adjusting the threshold so that it covers at least $50\%$ of {\small $R$}'s pixels. Regions in {\small $\hat{Y}$} that associate with high foreground probability values and overlap with {\small $R$} will be set as FG together with {\small $R$}. Similarly, regions with high background probabilities and that have no overlap with {\small $R$} will be assigned as BG. The remaining pixels are left as uncertain using the same distance criteria as in the 2D mask generation case and fed into GrabCut for lesion segmentation. In the limited cases where the CNN fails to detect any foreground regions, we generate {\small $\hat{T}$} solely from the estimated RECIST {\small $\hat{R}$}. We observe that when possible, GrabCut initialized by the CNN output performs better than being solely initialized from {\small $\hat{R}$}.

\textbf{Self-Paced CNN Training:} To generate 3D lesion segmentations from 2D RECIST annotations, we consider training the CNN in a self-paced or self-taught mechanism. It begins by learning the lesion appearances via CNN on RECIST-slices. After the model converges, {\small $Y=GrabCut(trimap(\hat{Y},\hat{R},R),X)$} is used to generate the training masks on successive slices so that it can be further fine-tuned with more ``harvested'' images. We progressively expand the extent of the harvested images, gradually expanding to include more CT slices along the longitudinal axis. Taking one lesion volume for example, the CNN is first trained on its RECIST slice {\small $X_{k}$} until convergence, we then apply this CNN model to slices {\small $[X_{k-\tau_{1}},X_{k+\tau_{1}}]$} to compute the predicted probability maps {\small $[\hat{Y}_{k-\tau},\hat{Y}_{k+\tau}]$}. Given these probability maps, we create \textit{trimaps} {\small $[\hat{T}_{k-\tau},\hat{T}_{k+\tau}]$} to employ GrabCut refinement \cite{khoreva_cvpr17_simpledoesit} on these slices. The GrabCut method consequently generates the training labels that are exploited for the CNN model training in the next round or iteration on {\small $[X_{k-\tau_{2}},X_{k+\tau_{2}}]$} slices. As this procedure proceeds iteratively, we can gradually obtain the converged lesion segmentation result in 3D. We summarize our WSSS method in Algorithm \ref{alg:wsss} and visually depict its process in Fig.~\ref{fig:overview}. Note that it is possible that {\small $GrabCut(\cdot)$} gives no or very few foreground areas or pixels if the initial \textit{trimap} and CT image are of bad quality. In these cases, we set up foreground, background and ignored uncertain pixels by combining the {\small $\hat{R}$} and the CNN output. CNN predicted foreground regions that overlap with {\small $\hat{R}$} will be assigned as foreground; predicted background regions that have no overlap with RECIST will be set as background; and the remaining pixels are ignored during training.

\begin{algorithm}[t!] \label{alg:wsss}
\caption{Self-Paced Weakly Supervised Segmentation}
\hspace*{\algorithmicindent} \textbf{Input} $D={(V^i,R^i)}$ for $i \in \{1, \ldots N\}$ , $K$, $\theta$.
\begin{algorithmic}[1]
\State $X^i = V^i(R^i)$, \hfill $\triangleright$ \textit{RECIST-Slice extraction}
\State $Y^i = GrabCut(trimap(R^i), X^i)$,
\State $\theta^0 := \min L(d,\theta)$, \hfill $\triangleright$ \textit{ConvNet training}
\State $k = 1$,
\For{$k \leq K $} \hfill $\triangleright$ \textit{Self-Paced ConvNet}
  \State $d = \emptyset$,
  \For {$i \in \{1, \ldots N\}$ and $\tau \in \{-r,\ldots,r\}$}
  \State $\hat{Y}^i_{k+\tau} = f(X^i_{k+\tau}, \theta^{k-1})$, \hfill $\triangleright$ \textit{ConvNet inference}
  \State $\hat{T}_{k+\tau} = Trimap(\hat{Y}^i_{k+\tau},\hat{R}^i_{k+\tau},R^i)$,
  \State $Y^i_{k+\tau} = GrabCut(\hat{T}_{k+\tau}, X^i_{k+\tau})$,
  \State $d = d + \{(X^i_{k+\tau}, Y^i_{k+\tau})\}$.
  \EndFor
\State $\theta^k := \min L(d,\theta^{k-1})$, \hfill $\triangleright$ \textit{ConvNet training}
\State $r = r + 1$.
\EndFor
\State \Return $\theta^K$
\end{algorithmic}
\end{algorithm}

%! TEX root=../main.tex
\subsection{Stacked-GAN Assisted Segmentation} \vspace{3mm}

We next investigate improving lesion segmentation accuracy by enhancing the quality and resolution of the input CT images via GANs. A direct implementation of super-resolution generative adversarial networks (SRGANs) \cite{ledig2016photo} on CT images produces many artificial, noisy edges and even deteriorates the final lesion segmentation outcome. Spurred by this observation, we propose a two-stage stacked GAN (SGAN) process that first reduces image noise and then performs object boundary enhancement. More specifically, each stage is conducted using an independent SRGAN \cite{ledig2016photo}. During model inference, the output of the first GAN will be fed as input to the second GAN. For lesion segmentation, we use both the denoised and enhanced outputs from SGAN and the original CT image as three-channel inputs since they may contain complementary information.

\textbf{Synthesized Training Data:} Normally the SGAN or SRGAN models are trained with pairs of low- and high-resolution images. This can be obtained easily in natural images (by down-sampling). However physical CT images are imaged by medical scanners at roughly fixed in-plane resolutions of $\sim1$ mm per-pixel and CT imaging at ultra-high spatial resolutions does not exist. 
For the sake of SGAN training, we leverage transfer learning using a large-scale synthesized natural image dataset: DIV2K \cite{agustsson_2017_cvpr_workshops} where all images are converted into gray scale and down-sampled to produce training pairs. For the training of the denoising GAN, we randomly crop {\small $32\times32$} sub-images from distinct training images of DIV2K. White Gaussian noise at different variance levels {\small $\sigma\in(0,50]$} are added to the cropped images to construct the paired model inputs. For training the image-enhancement GAN, the input images are cropped as {\small $128\times128$} patches and we perform the following steps: 1) down-sample the cropped image with scale {\small $s\in[1,4]$}, 2) implement Gaussian smoothing with {\small $\sigma\in(0,3]$}, 3) execute contrast compression with rates of {\small $\kappa\in[1,3]$}, and 4) conduct up-sampling with the scale {\small $s$} to generate images pairs.


==> sections/method_Adam.tex <==
%!TEX root=../main.tex
\begin{figure*}[t!]
\begin{center}
   \includegraphics[width=0.96\linewidth]{figures/OverView2.pdf}
\end{center}
\vspace{-4mm}
\caption{Our weakly supervised deep lesion segmentation framework. We use CNN output to gradually generate extra training data for self-paced learning. Regions colored with red, orange, green, and blue inside the \textit{trimap} present FG, PFG, PBG, and BG in respective.}
\label{fig:overview}
\end{figure*}

%-------------------------------------------------------------------------
In DeepLesion dataset \cite{yan_2017_deep-lesion}, manually selected axial CT slices contain RECIST diameters that represent the longest axis and its perpendicular counterpart. Given RECIST diameters as weak supervision, we leverage WSSS principles to learn a deep lesion CNN segmentation model using both 2D slice and 3D volumes with no extra pixel-wise manual annotations. Our pipeline for WSSS contains four main steps as follows. %% %%: 1) converting RECIST diameters to training masks, 2) learning a 2D CNN lesion appearance model, 3) expanding the 2D model into 3D segmentation, and optionally 4) using SGAN to generate enhanced images as input. 

\subsection{From RECIST to 2D Training Masks} \label{sec:init-mask}
We denote elements in the DeepLesion dataset \cite{yan_2017_deep-lesion} as {\small $\mathcal{D}=\{(V^i,R^i)\}$} for {\small $i \in \{1,\ldots,N\}$}, where {\small $N$} is the number of lesions, {\small $V^i$} is the CT region of interest, and {\small $R^i$} is the corresponding RECIST diameters. To create the 2D training data for the WSSS model, the image and label map pairs, {\small $X^i$} and {\small $Y^i$}, respectively, must be generated. Together they comprise the set {\small $\mathcal{F}=\{(X^i, Y^i)\}$}, for {\small $i \in \{1,\ldots,N\}$}. For notational clarity, we drop the superscript $i$. {\small $X=V_{r}$} is simply the RECIST-slice, \ie{}, the axial slice that contains {\small $R$}, and $r$ is its slice number. Both GrabCut \cite{rother_2004_grabcut} and densely-connected conditional random fields (DCRF) \cite{krah_2012_fully-crf} can be adopted to produce the training mask $Y$. When GrabCut starts with a good quality initial \textit{trimap} (explained below), we observe that it produces better results, which is consistent with the findings in \cite{khoreva_cvpr17_simpledoesit}.

More specifically, GrabCut is initialized with the image foreground and background regions and produces a segmentation using iterative energy minimization. Good initializations located near the global energy minimum may aid GrabCut's convergence. We use the spatial prior information, provided by {\small $R$}, to compute a high quality initial \textit{trimap} {\small $T$} from {\small $R$}, \ie{}, regions of probable background (PBG), probable foreground (PFG), background (BG), and foreground (FG)~\cite{rother_2004_grabcut}. Note that unlike the original \textit{trimap} definition, we define four region types. More specifically, if the lesion bounding box tightly around the RECIST axes is $[w,h]$, a $[2w,2h]$ ROI is cropped from the RECIST-slice. The \textit{trimap} assigns the outer $50\%$ as BG and allocates $10\%$ of the image region, dilated from {\small $R$} as FG. The remaining $40\%$ is divided in half between PFG and PBG based on the distances to FG and BG. Finally, the long/short axes of $R$ roughly clamp the size of GrabCut segmentation, ensuring that the segmentation will not shrink into a small region when the CT image intensity distribution is homogeneous and no clear lesion boundary is presented. Fig.~\ref{fig:overview} visually depicts the mask generation process.

%-------------------------------------------------------------------------
\subsection{CNN Lesion Appearance Model}

Many image classification or segmentation CNN models have been presented in recent works \cite{simonyan_2014_vggnet,he_2016_resnet,huang_2017_densenet,xie_2015_hnn,ronneberger_2015_unet}. Without loss of generality, we use the holistically-nested network (HNN) \cite{xie_2015_hnn} and UNet \cite{ronneberger_2015_unet} as our baselines, both of which provide state-of-the-art, yet straightforward semantic architectures. We represent our CNN models as a mapping function {\small $\hat{Y} = f(X;\theta)$}, with the goal of optimizing {\small $\theta$} to minimize the differences between the current model outputs {\small $\hat{Y}$} and ground truth training labels {\small $Y$}. Although the GrabCut masks are imperfect, we use them as {\small $Y$} for the next step of CNN model training, expecting that the CNN will generalize well even with considerable label noise. Thus, we aim to minimize
\begin{equation} \label{eq:convnet}
	L(\mathcal{F}; \theta) = \frac{1}{N} \sum\limits_{i=1}^{N} \frac{\sum\limits_{m\in Y^i} H (\hat{y}^{(i,m)},y^{(i,m)})}{|Y^i|} \textrm{,}
\end{equation}
where {\small $m$} is the pixel index inside {\small $Y$}, {\small $|Y|$} is the cardinality of {\small $Y$}, and {\small $H(\cdot)$} is the cross-entropy function. 

%-------------------------------------------------------------------------
\subsection{Self-Pacing for Volume Segmentation} \label{sec:3d-wsss}

For obtaining 3D volume segmentations, we follow a similar strategy as with the RECIST slices, except in the 3D case, we must infer $R$ for off-RECIST slices and also incorporate inferences from the CNN model. These two priors are used together for self-paced CNN training.

\textbf{3D RECIST Estimation:} A simple way to generate off-RECIST-slice  {\small $R$} diameters is to take advantage of the fact that RECIST-slice {\small $R$}'s lie on the maximal cross-sectional area of the lesion. The rate of reduction of off-RECIST-slice endpoints is then calculated by their relative distance to the intersection point of the major and minor axes. Estimated 3D RECIST endpoints are then projected from the actual RECIST endpoints by Pythagorean theorem using physical Euclidean distance.

\textbf{Trimap from CNN Output:} Different from Sec.~\ref{sec:init-mask}, \textit{trimap} generation now takes both the CNN output {\small $\hat{Y}$} and the estimated RECIST {\small $\hat{R}$} as inputs: {\small $\hat{T} = trimap(\hat{Y},\hat{R},R)$}. The {\small $\hat{Y}$} is first binarized by adjusting the threshold so that it covers at least $50\%$ of {\small $R$}'s pixels. Regions in {\small $\hat{Y}$} that associate with high foreground probability values and overlap with {\small $R$} will be set as FG together with {\small $R$}. Similarly, regions with high background probabilities and that have no overlap with {\small $R$} will be assigned as BG. The remaining pixels are left as uncertain using the same distance criteria as in the 2D mask generation case and fed into GrabCut for lesion segmentation. In the limited cases where the CNN fails to detect any foreground regions, we generate {\small $\hat{T}$} solely from the estimated RECIST {\small $\hat{R}$}. We observe that when possible, GrabCut initialized by the CNN output performs better than being solely initialized from {\small $\hat{R}$}.

\textbf{Self-Paced CNN Training:} To generate 3D lesion segmentations from 2D RECIST annotations, we train the CNN model in a self-paced or self-taught mechanism. It begins by learning the lesion appearances via CNN on RECIST-slices. After the model converges, {\small $Y=GrabCut(trimap(\hat{Y},\hat{R},R),X)$} is used to generate the training masks on successive slices so that it can be further fine-tuned on more newly ``harvested'' images. We progressively expand the extent of the harvested images, to include more CT slices along the longitudinal axis. Taking one lesion volume for example, the CNN is first trained on its RECIST slice {\small $X$} until convergence, we then apply this CNN model to slices {\small $[V_{r-1},V_{r+1}]$} to compute the predicted probability maps {\small $[\hat{Y}_{r-1},\hat{Y}_{r+1}]$}. Given these probability maps, we create \textit{trimaps} {\small $[\hat{T}_{r-1},\hat{T}_{r+1}]$} to employ GrabCut refinement \cite{khoreva_cvpr17_simpledoesit} on these slices. The GrabCut method consequently generates the training labels that are used by the CNN model in the next training round on the slices {\small $[V_{r-2},V_{r+2}]$} slices. As this procedure proceeds iteratively, we can gradually obtain the converged lesion segmentation result in 3D. We summarize our WSSS method in Algorithm~\ref{alg:wsss} and visually depict its process in Fig.~\ref{fig:overview}. Note that it is possible that {\small $GrabCut(\cdot)$} gives no or very few foreground areas or pixels if the initial \textit{trimap} and CT image are of bad quality. In these cases, we set up foreground, background and ignored uncertain pixels by combining the {\small $\hat{R}$} and the CNN output. CNN predicted foreground regions that overlap with {\small $\hat{R}$} are assigned as foreground; predicted background regions that have no overlap with RECIST are set as background; with the remaining pixels ignored during training.

\begin{algorithm}[t!] 
	\caption{Weakly Supervised Self-Paced CNN Training} \label{alg:wsss}
	\textbf{Input:} $\mathcal{D}={(V^i,R^i)}$ for $i \in \{1, \ldots N\}$  \hfill $\triangleright$ \textit{Deep-Lesion dataset}
	\textbf{Input:} \textit{3D RECIST Estimation:} $\hat{R}^i$ \\
	\textbf{Input:} \textit{Maximum iteration:} $K$, \textit{initial CNN model:} $\theta$.
	\begin{algorithmic}[1]
		\State $X^i = V^i_r$ \hfill $\triangleright$ \textit{RECIST-Slice extraction}
		\State $Y^i = GrabCut(trimap(R^i), X^i)$ \hfill $\triangleright$ \textit{Initial Train-Mask}
		\State $\mathcal{F} = \{(X^i,Y^i)\}$ \hfill $\triangleright$ \textit{RECIST-slices training set}
		\State $\theta^0 := \min L(\mathcal{F},\theta)$ \hfill $\triangleright$ \textit{Training of initial 2D segmentation}
		\For{$k=1$ to $K$}
		\State $\mathcal{F} = \emptyset$
		\For {$\tau=-k$ to $k$}
		\State $\hat{Y}^i_{r+\tau} = f(V^i_{r+\tau}, \theta^{k-1})$, \hfill $\triangleright$ \textit{CNN inference}
		\State $\hat{T}_{r+\tau} = trimap(\hat{Y}^i_{r+\tau},\hat{R}^i_{r+\tau},R^i)$,
		\State $Y^i_{r+\tau} = GrabCut(\hat{T}_{r+\tau}, V^i_{r+\tau})$,
		\State $\mathcal{F} = \mathcal{F} \cup \{(V^i_{r+\tau}, Y^i_{r+\tau})\}$.
		\EndFor
		\State $\theta^k := \min L(\mathcal{F},\theta^{k-1})$, \hfill $\triangleright$ \textit{CNN training with multi-slices}
		\EndFor \\
		\Return $\theta^K$ \hfill $\triangleright$ \textit{Return trained CNN model}
	\end{algorithmic}
\end{algorithm}
%! TEX root=../main.tex
\subsection{Stacked-GAN Assisted Segmentation}

We next investigate improving lesion segmentation accuracy by enhancing the quality and resolution of the input CT images via GANs. A direct application of super-resolution generative adversarial networks (SRGANs) \cite{ledig2016photo} on CT images produces many artificial, noisy edges and even deteriorates the final lesion segmentation outcome. Spurred by this observation, we propose a two-stage stacked GAN (SGAN) process that first reduces image noise and then performs object boundary enhancement. More specifically, each stage is conducted using an independent SRGAN \cite{ledig2016photo}. During model inference, the output of the first GAN will be fed as input to the second GAN. For lesion segmentation, we use both the denoised and enhanced outputs from SGAN and the original CT image as three-channel inputs since they may contain complementary information.

\textbf{Synthesized Training Data:} Normally the SGAN or SRGAN models are trained with pairs of low- and high-resolution images. This can be obtained easily in natural images (by down-sampling). However physical CT images are imaged by medical scanners at roughly fixed in-plane resolutions of $\sim1$ mm per-pixel and CT imaging at ultra-high spatial resolutions does not exist. 
For the sake of SGAN training, we leverage transfer learning using a large-scale synthesized natural image dataset: DIV2K \cite{agustsson_2017_cvpr_workshops} where all images are converted into gray scale and down-sampled to produce training pairs. For the training of the denoising GAN, we randomly crop {\small $32\times32$} sub-images from distinct training images of DIV2K. White Gaussian noise at different variance levels {\small $\sigma\in(0,50]$} are added to the cropped images to construct the paired model inputs. For training the image-enhancement GAN, the input images are cropped as {\small $128\times128$} patches and we perform the following steps: 1) down-sample the cropped image with scale {\small $s\in[1,4]$}, 2) implement Gaussian smoothing with {\small $\sigma\in(0,3]$}, 3) execute contrast compression with rates of {\small $\kappa\in[1,3]$}, and 4) conduct up-sampling with the scale {\small $s$} to generate images pairs.

To fine-tune using CT images, we process $28,000$ training RECIST slices using the current trained SGAN and select a subset of up to $1,000$ slices by subjectively inspecting the CT super-resolution results. The selected CT images are subsequently added to the training for the next round of SGAN fine-tuning. This iterative process finishes when no more visual improvement could be observed.


==> sections/related-work.tex <==
%!TEX root=../main.tex
%-------------------------------------------------------------------------
WSSS is a challenging computer vision task that has drawn considerable interest. Recently promising results have been reported \cite{d_pap_iccv17_extreneclick,khoreva_cvpr17_simpledoesit,d_lin_cvpr16_scribblesup,g_papandreou_iccv15_wssl,j_dai_iccv15_boxsup,bearman_2015_pointsegment,wei_2015_stc,hong_2017_wsssweb}. Most WSSS methods update pixel labels and CNN models using training iterations. The pixel-level training label is often initialized from weak annotations, \eg{}, bounding boxes of foreground objects. Subsequently, CNNs are trained to capture the initial masks. Although many pixels are possibly initially mislabelled, the CNNs are expected to robustly handle label noise (to some extent) and model the complete data distribution. Once the CNN model converges, its output is used to obtain more accurate pixel labels. Updates between CNN and pixel training labels loop iteratively until no further changes can be measured. However, as observed in \cite{khoreva_cvpr17_simpledoesit}, very high-quality initial pixel labels can allow the CNN model to converge in as few as $1\sim2$ iterations.

Thus, it is essential to have the object mask ``correctly'' initialized and updated. A popular mask initialization uses multiscale combinatorial grouping (MCG)~\cite{j_pt_tpami17_mcg} to group superpixels into plausible object parts, using a bounding box to delineate foreground, background, and uncertain regions during CNN training~\cite{j_dai_iccv15_boxsup, khoreva_cvpr17_simpledoesit}. RECIST diameters are similar to scribbles over foreground objects, and these can be used to coarsely delineate superpixels into foreground and background~\cite{d_lin_cvpr16_scribblesup}. However, empirically MCG does not perform well under the CT imaging modality (compared to natural images) and thus is not suitable for our lesion segmentation task. Semantic edge based methods, like GrabCut$^+$ \cite{khoreva_cvpr17_simpledoesit, d_pap_iccv17_extreneclick}, are also not applicable because unsupervised edge detection methods, such as gPb \cite{j_pt_tpami17_mcg}, suffer from abundant false positives or perform unstably across the whole CT image dataset. %Similarly, GrabCut \cite{khoreva_cvpr17_simpledoesit} and dense Conditional Random Field (DCRF) \cite{g_papandreou_iccv15_wssl} can replace MCG sometimes, or in the extreme case that simply setting the center of the bounding box as foreground (i.e., low recall) where training with high precision object labels is found to be beneficial \cite{khoreva_cvpr17_simpledoesit}, for train CNNs under weak supervision.
%On the contrary, direct pixel-level GrabCut \cite{rother_2004_grabcut, khoreva_cvpr17_simpledoesit} is found to be able to generate the initial object training label maps of high quality, especially when the {\textit{Trimap}} \cite{rother_2004_grabcut} is carefully generated. %But good training label can not be generated for the lesion volume at the very beginning, iterative updating between training label and CNN is still implemented in our work. %DCRF \cite{krah_2012_fully-crf} is successful in natural image segmentation, but in CT images, pixel value in lesion is sometimes similar to objects in the background so that DCRF fails to deliver promising lesion segmentation with many false positive be produced.
Another stream of related work is extending WSSS from static images to video~\cite{hong_2017_wsssweb}. In videos, the same object often retains similar appearance across different temporal frames even though the locations may vary. Using this prior, the training images of object-wise labels can be extracted and propagated across video frames to facilitate CNN training. %However, in our lesion segmentation task, the ImageNet pre-trained appearance CNN models \cite{Deng2009ImageNet,simonyan_2014_vggnet,he_2016_resnet} to detect common object in image sequences are not applicable. 
However lesions exhibit not only positional movements but also drastic morphological changes across CT slices, adding further challenges to lesion volume segmentation from RECIST diameters. Hence, our work differs from prior art by employing a principled GrabCut~\cite{rother_2004_grabcut} and \textit{trimap} mask initialization, coupled with self-paced learning~\cite{kumar_2010_sp-svm} to progressively refine the 3D lesion segmentations. % than processing WSSS in the videos of nature objects.

Recently, deep CNN based image super-resolution methods \cite{dong2016image,kim2016accurate,kim2016deeply,ledig2016photo,sajjadi2016enhancenet,shi2016real,johnson2016perceptual,lai2017deep,taiimage2017,tong2017image,dahl2017pixel} have achieved state-of-the-art performance, due to CNN's capability to learn powerful features and model long-range contextual information from a collection of low resolution images. Mappings between low and high resolution images are learned by minimizing the mean squared error (MSE) loss or perceptual loss \cite{johnson2016perceptual,ledig2016photo,sajjadi2016enhancenet}. Adversarial learning strategies \cite{ledig2016photo} are also employed to train CNN models for better reconstruction of fine details and edges. In this work, we adopt the perceptual loss and adversarial learning to simulate high-resolution images ($\sim0.2$ mm per-pixel) via CNNs directly from the original CT images ($\sim1.0$ mm per-pixel). Unlike other works, we use the enhanced images to improve the WSSS performance.

%No low- and high-resolution image pairs are available for training.


==> sections/related-work_Le.tex <==
%!TEX root=../main.tex
%-------------------------------------------------------------------------
WSSS is a challenging computer vision task that has drawn considerable interest. Recently promising results have been reported \cite{d_pap_iccv17_extreneclick,khoreva_cvpr17_simpledoesit,d_lin_cvpr16_scribblesup,g_papandreou_iccv15_wssl,j_dai_iccv15_boxsup,bearman_2015_pointsegment,wei_2015_stc,hong_2017_wsssweb}. Most WSSS methods update pixel labels and CNN models using training iterations. The pixel-level training label is often initialized from weak annotations, \eg{}, bounding boxes of foreground objects. Subsequently, CNNs are trained to capture the initial masks. Although many pixels are possibly initially mislabelled, the CNNs are expected to robustly handle label noise (to some extent) and model the complete data distribution. Once the CNN model converges, its output is used to obtain more accurate pixel labels. Updates between CNN and pixel training labels loop iteratively until no further changes can be measured. However, as observed in \cite{khoreva_cvpr17_simpledoesit}, very high-quality initial pixel labels can allow the CNN model to converge in as few as $1\sim2$ iterations.

Thus, it is essential to have the object mask ``correctly'' initialized and updated. A popular mask initialization uses multiscale combinatorial grouping (MCG)~\cite{j_pt_tpami17_mcg} to group superpixels into plausible object parts, using a bounding box to delineate foreground, background, and uncertain regions during CNN training~\cite{j_dai_iccv15_boxsup, khoreva_cvpr17_simpledoesit}. RECIST diameters are similar to scribbles over foreground objects, and these can be used to coarsely delineate superpixels into foreground and background~\cite{d_lin_cvpr16_scribblesup}. However, empirically MCG does not perform well under the CT imaging modality (compared to natural images) and thus is not suitable for our lesion segmentation task. Semantic edge based methods, like GrabCut$^+$ \cite{khoreva_cvpr17_simpledoesit, d_pap_iccv17_extreneclick}, are also not applicable because unsupervised edge detection methods, such as gPb \cite{j_pt_tpami17_mcg}, suffer from abundant false positives or perform unstably across the whole CT image dataset. %Similarly, GrabCut \cite{khoreva_cvpr17_simpledoesit} and dense Conditional Random Field (DCRF) \cite{g_papandreou_iccv15_wssl} can replace MCG sometimes, or in the extreme case that simply setting the center of the bounding box as foreground (i.e., low recall) where training with high precision object labels is found to be beneficial \cite{khoreva_cvpr17_simpledoesit}, for train CNNs under weak supervision.
%On the contrary, direct pixel-level GrabCut \cite{rother_2004_grabcut, khoreva_cvpr17_simpledoesit} is found to be able to generate the initial object training label maps of high quality, especially when the {\textit{Trimap}} \cite{rother_2004_grabcut} is carefully generated. %But good training label can not be generated for the lesion volume at the very beginning, iterative updating between training label and CNN is still implemented in our work. %DCRF \cite{krah_2012_fully-crf} is successful in natural image segmentation, but in CT images, pixel value in lesion is sometimes similar to objects in the background so that DCRF fails to deliver promising lesion segmentation with many false positive be produced.
Another stream of related work is extending WSSS from static images to video~\cite{hong_2017_wsssweb}. In videos, the same object often retains similar appearance across different temporal frames even though the locations may vary. Using this prior, the training images of object-wise labels can be extracted and propagated across video frames to facilitate CNN training. %However, in our lesion segmentation task, the ImageNet pre-trained appearance CNN models \cite{Deng2009ImageNet,simonyan_2014_vggnet,he_2016_resnet} to detect common object in image sequences are not applicable. 
However lesions exhibit not only positional movements but also drastic morphological changes across CT slices, adding further challenges to lesion volume segmentation from RECIST diameters. Hence, our work differs from prior art by employing a principled GrabCut~\cite{rother_2004_grabcut} and \textit{trimap} mask initialization, coupled with self-paced learning to progressively refine the 3D lesion segmentations. % than processing WSSS in the videos of nature objects.

Recently, deep CNN based image super-resolution methods \cite{dong2016image,kim2016accurate,kim2016deeply,ledig2016photo,sajjadi2016enhancenet,shi2016real,johnson2016perceptual,lai2017deep,taiimage2017,tong2017image,dahl2017pixel} have achieved state-of-the-art performance, due to CNN's capability to learn powerful features and model long-range contextual information from a collection of low resolution images. Mappings between low and high resolution images are learned by minimizing the mean squared error (MSE) loss or perceptual loss \cite{johnson2016perceptual,ledig2016photo,sajjadi2016enhancenet}. Adversarial learning strategies \cite{ledig2016photo} are also employed to train CNN models for better reconstruction of fine details and edges. In this work, we adopt the perceptual loss and adversarial learning to simulate high-resolution images ($\sim0.2$ mm per-pixel) via CNNs directly from the original CT images ($\sim1.0$ mm per-pixel). Unlike other works, we use the enhanced images to improve the WSSS performance.

%No low- and high-resolution image pairs are available for training.

